Fine-grained Classification of Rowing teams

Fine-grained classification tasks such as identifying different breeds of dog are quite challenging as visual differences between categories is quite small and can be easily overwhelmed by external factors such as object pose, lighting, etc. This work focuses on the specific case of classifying rowing teams from various associations. Currently, the photos are taken at rowing competitions and are manually classified by a small set of members, in what is a painstaking process. To alleviate this, Deep learning models can be utilised as a faster method to classify the images. Recent studies show that localising the manually defined parts, and modelling based on these parts, improves on vanilla convolution models, so this work also investigates the detection of clothing attributes. The networks were trained and tested on a partially labelled data set mainly consisting of rowers from multiple associations. This paper resulted in the classification of up to ten rowing associations by using deep learning networks the smaller VGG network achieved 90.1\% accuracy whereas ResNet was limited to 87.20\%. Adding attention to the ResNet resulted into a drop of performance as only 78.10\% was achieved.

==> tables/01_fashion.tex <==
\begin{table}[ht!]
    \centering
    \caption{Clothing Datasets}
    \begin{tabular}{lr} \toprule
        
        Fashionista dataset & \cite{yamaguchi2012parsing} \\ 
        Clothing Attributes Dataset & \cite{chen2012describing} \\ 
        Paper Doll & \cite{yamaguchi2013paper}  \\ 
        Color-Fashion Dataset & \cite{liu2013fashion}  \\ 
        MVC Dataset & \cite{liu2016mvc} \\ 
        Deep Fashion Dataset & \cite{liuLQWTcvpr16DeepFashion} \\ 
        Fashion Mnist & \cite{xiao2017/online} \\ 
        imat fashion & \cite{iMaterialist} \\ \bottomrule
    \end{tabular}
    \label{tab:clothingdatasets}
\end{table}

==> tables/02_clothingdataset.tex <==
\begin{table}[ht!]
    \centering
    \caption{Clothing Data sets}
    \label{tab:clothingdatasets}
    \begin{tabular}{lr}
        \toprule
        Name                            & Citation \\ 
        \midrule
        Fashionista data set            & \cite{yamaguchi2012parsing} \\ 
        Clothing Attributes Data set    & \cite{chen2012describing} \\ 
        Paper Doll                      & \cite{yamaguchi2013paper}  \\ 
        Color-Fashion Data set          & \cite{liu2013fashion}  \\ 
        MVC Dataset                     & \cite{liu2016mvc} \\ 
        Deep Fashion Data set           & \cite{liuLQWTcvpr16DeepFashion} \\ 
        Fashion-MNIST                   & \cite{xiao2017/online} \\ 
        imat fashion                    & \cite{iMaterialist} \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> tables/03_accuracy_Data_set.tex <==
\begin{table}[ht!]
    \centering
    \caption{Accuracy of the data set}
    \label{tab:data_exp}
    \begin{tabular}{cc}
    \toprule
    Association & Accuracy [\%] \\ \midrule
    Argo & 86.0 \\ 
    Gyas & 85.8 \\ 
    Laga & 91.1 \\
    Nereus & 83.0 \\
    Njord & 79.1 \\
    Orca & 86.0 \\
    \pe & 97.1 \\
    Skadi & 68.7 \\
    Skoll & 84.0 \\
    Triton & 100 (already cleaned) \\ \bottomrule
    \end{tabular}
\end{table}

==> tables/03_performances_datasets.tex <==

\begin{table}[ht!]
\centering
\caption{Data set v3 vs v5}
\begin{tabular}{lcc} \toprule
\textbf{Dataset}                                                     & \textbf{Val acc [\%]} & \textbf{Test acc [\%]}   \\ \midrule
roeiboat-v3          & 90.09                                         & 87.40                                            \\
roeiboat-v5          & 95.46                                         & 90.10                                            \\ \hline
% Training set = v5, validation set = v3         & 94.56                                         & 90.10                                            \\ \hline
\end{tabular}
\label{table:v5_vs_v3}
\end{table}

